In-Distribution Interpretability for Challenging Modalities

It is widely recognized that the predictions of deep neural networks are difficult to parse relative to simpler approaches. However, the development of methods to investigate the mode of operation of such models has advanced rapidly in the past few years. Recent work introduced an intuitive framework which utilizes generative models to improve on the meaningfulness of such explanations. In this work, we display the flexibility of this method to interpret diverse and challenging modalities: music and physical simulations of urban environments.

==> sections/broaderimpact.tex <==
\section*{Broader Impact}
\memo{Possibility of going beyond images, maybe medical applications.} RL, GNN for chemistry, ..

==> sections/experiments.tex <==
\section{Experiments on Radio Maps}

%\subsection{Interpreting Radio Map Generation Methods}

We demonstrate the flexibility of our approach on the problem of interpreting deep learning based physical simulations. In these problems, a network is trained with supervision to match the outcome of a physical simulation given the initial configuration. Once trained, these simulators typically have two advantages over their physical counterparts: they are more efficient computationally and they are guaranteed to produce an outcome after a set amount of computations.

\subsection{RadioUNet Methods}

The particular simulation we consider is that of estimating radio maps in urban environments. We have a device Tx transmitting a signal in some part of a city. The received signal strength varies with the location and depends on the physical factors like line of sight obstacles, reflection, and diffraction. The problem is to estimate the function that assigns the proper strength of the signal to each location in the city. The associated dataset is the RadioMapSeer dataset \cinjon{cite} consisting of 700 city maps, 80 transmitter locations per map, and a corresponding grayscale radio map label.

We consider the following setting from [*]\cite{Ron, is this from some other paper?} \textcolor{blue}{(Ron) same paper}. We receive as input a perturbed map of the city, along with some measurements of the target radio map at a few locations. For the perturbation, we suppose that a few buildings are missing in each map.
The architecture, called RadioUNet$_S$ ($S$ for samples), is interpreted as a hybrid interpolation-simulation method, which interpolates \cosmas{what does that mean?} the measurements and uses the perturbed city map to guide the output to be physically feasible\cinjon{Ron, is this just augemntation of the data?}\textcolor{blue}{(Ron) I am not sure what you mean. The method computes a physical simulation based on the map, but also uses the measurements.}. 
RadioUNet$_S$ is a CNN that receives as inputs three channels, the binary map of the city (white inside buildings and black outside), the binary map of Tx (white at the location of Tx and black elsewhere), and the measurements as a gay level image with the strength of the signal at the measured locations and zero elsewhere. RadioUNet$_S$ outputs one channel -- the estimation of the radio map. We also consider a simpler CNN from [*]\cite{Ron, ditto ... is this from some other paper?}\textcolor{blue}{(Ron) same paper}, called RadioUNet$_C$ ($C$ for clean), which only receives the map and Tx as inputs, and is trained with accurate city maps \cosmas{which maps?}\Ron{Do you think it is not clear that I use the same dataset?} \cosmas{I think the distinction between city maps and radio maps should be more obvious}. For an example of a ground truth radio map and its estimations via RadioUNet$_S$ and RadioUNet$_C$ see Figures \ref{fig:radio1}, \ref{fig:radio2}, and \ref{fig:radio4} respectively.

\subsection{Explaining RadioUNet Methods}

In Figures \ref{fig:radio1} and \ref{fig:radio2},  an example ground truth and estimated radio map via RadioUNet$_S$ are shown. Observe that the network in-fills the missing building with a shadow. As a black box method, it is unclear what lead the network to react this way to the input domain. Understanding why the network did this is important if the method is to be transferred to real-life deployment; the model might have learned subtleties that work for this dataset that will not work more broadly in real cities .
For example, since in every map some buildings are taken out, it is possible that the network learned to inpaint them back relying on patterns in the map of the city itself. Such a network is likely to fail in real life, where the sources of perturbation are more extensive (e.g. vegetation and cars). 
We would thus like to know whether measurements or buildings are more influential to the model in certain areas, such as in the vicinity of a missing building.

%For example, since in every map some buildings are taken out, the network can learn to inpaint them back relying on patterns in the city map itself. Such a behavior is undesirable, since the sources of perturbation in real-life deployment are more diverse then a mere deletion of buildings, including, e.g., vegetation and  cars. More generally, the perturbation can be seen as any discrepancy between the physical simulation and the real-life phenomenon. 
%
%To promote transferability, the input measurements, rather than patterns in the city, should help guide RadioUNet$_S$ to match the ground truth in places where RadioUNet$_C$ fails.
%We would thus like to know what information is more influential, measurements or buildings, for the generation of the radio map in some area of interest in the map, like the vicinity of a missing building.



%REMARK: instead of hand picking the odmain of interest, take the difference between RadioUNet$_C$ and RadioUNet$_S$, and explain discrepency between them - namely, the difference is a continuous map that focuses the interpretation.

We hence consider the simple paradigm of relevance maps, in which each building and measurement is one piece of information. We optimize the relevance map using matching pursuit (MP) \cosmas{Needs more explanation if not given in other sections} \Ron{We should define the MP approach before.} and define the completion of the transmitted data as follows. For buildings, since the goal is to query whether or not the input map is inpainted in RadioUNet$_S$, it is important to avoid inpainting in the completion step. Indeed, inpainting the transmitted partial city relieves RadioUNet$_S$ of this task. Note that any subset of buildings in a city map is a valid city map on its own, and RadioUNet methods perform well in such partial cities. 

For the measurements, we consider two extreme cases. First, the chosen subset of measurements is kept unchanged, and unchosen measurements are simply set to zero. Indeed, any subset of measurements is a valid set of measurements on it own. In the other extreme, we inpaint the unchosen measurements using another physical simulation. For this, we estimate the radio map using RadioUNet$_C$ based on the chosen buildings. We then sample this estimation at the locations of the unchosen measurements to obtain the inpainting. \cosmas{I don't get it}\Ron{How about now?} Between these two extremes there is a continuum of completion methods where a random subset of the unchosen measurements are sampled from RadioUNet$_C$, with probability between 0 and 1, and the rest are not taken as measurements (set to zero).

The two extreme measurement completion methods represent two extremes of the interpretation query. Sampling values from RadioUNet$_C$ to fill in the missing measurements tends to overestimate the strength of the signal since only the relevant buildings are used in the RadioUNet$_C$ simulation.  Choosing no measurements and no buildings will complete all measurements to the maximal possible signal strength -- the free space radio map. The overestimation in the signal strength is reduced the more measurements and buildings are transmitted, resulting in darker estimated radio maps.
This query can be thus dubbed as ``which measurements and buildings are important in order to darken the free space radio map, turning it to the radio map produced by RadioUNet$_S$?''

On the other extreme, zeroing out non-transmitted measurements tends to create darker radio maps. Hence, this query can be dubbed as ``when synthesizing radio maps by filling in bright spots, which measurements and buildings are most important?''  
This phenomenon occurs as a result of the implementation of the measurement campaign. In training, random points in the map are sampled uniformly, and discarded if they happen to be inside a building. As a result, the network learns that a patch of the map, lacking any measurement, is likely to indicate a location of a building. Hence, when measurements are chosen to be transmitted, and form a ``non-uniform spatial pattern'', the network tends to fill in large patches lacking of measurements with dark shadows. In fact, this observation is already a first insight provided by our interpretability approach. By seeing the relevant information produced in MP, and the radio map computed from this information, we could simultaneously identify the  problem with uniform measurements and dub the interpretation query as ``what is relevant for filling in bright spots.''  

An example explanation using the two extreme queries is presented in Figure \ref{fig:radio_queries}. We construct an explanation for an area of interest about the location of a missing building. Note that RadioUNet is based on compositions of UNets, and is thus interpreted as a procedure of extracting high level and global information from the inputs to synthesize the output. The chosen buildings in Figure \ref{fig:radio_queries} reflect the global nature of the RadioUNet method.

\begin{figure}
	\centering
	\begin{subfigure}{0.32\textwidth}\centering%no!\hfill
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/3_estimate_all.png}
		\caption{Estimated radio map. \newline\newline}
		\label{fig:radio_queries1}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.32\textwidth}\centering
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/3_explanation_all2.png}
		\caption{Explanation via inpainting all unchosen measurements with RadioUNet$_C$.}
		\label{fig:radio_queries2}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.32\textwidth}\centering
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/3_explanation_2_5_p2.png}
		\caption{Explanation via inpainting 2.5\% of the unchosen measurements with RadioUNet$_C$.}
	   \label{fig:radio_queries3}
	\end{subfigure}%
	\caption{Radio map queries and explanations. Gray: radio map. Blue: input buildings. Red: input measurements. Green: interpretation area of interest. Middle: since the query is how to fill in the image with shadows, samples in the shadow of the missing building are the most influential for RadioUNet$_S$. Right: since the query is how to fill in the image both with shadows and bright spots, both samples in the shadow of the missing building and samples right before the building, in the line-of-sight of Tx, are the most influential for RadioUNet$_S$.}
	\label{fig:radio_queries}
\end{figure}

\subsection{Example Application: Interpretation Driven Training}

In this subsection we consider the interpretation query based on inpainting all unchosen measurements with RadioUNet$_C$.
%
As discussed above, when a missing building is in line-of-sight of Tx, we would like RadioUNet$_S$ to reconstruct this building relying on samples in the shadow of the building rather than patterns in the map of the city. 
To reduce the reliance of RadioUNet$_S$ on the map information in this situation, we add a loss term in training which promotes measurement explanations. To check if the missing building is in line-of-sight, we compute RadioUNet$_C$ of the input map, which misses some buildings. If the building is in line-of-sight, than the minimal  value of the RadioUNet$_C$ simulation inside the missing building must be high. Thus, the interpretation loss is taken to be non-zero only if this minimum is higher than some fixed value, e.g., $0.3$. In this case, we compute RadioUNet$_S$ based only on the measurements, with no buildings input, and define the interpretation loss as (negative) the $l_2$ distance between the outputs of RadioUNet$_S$ with buildings$+$measurements  and RadioUNet$_S$ with measurements alone, restricted to the missing building. After training, the explanation around missing buildings tend to rely more on measurements in the shadow of the buildings than before, and less on buildings (see Figure \ref{fig:radio}).


\begin{figure}
	\centering
	\begin{subfigure}{0.32\textwidth}\centering%no!\hfill
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/7_targer.png}
		\caption{Ground Truth Radio Map \newline}
		\label{fig:radio1}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.32\textwidth}\centering
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/7_estimate.png}
		\caption{Standard RadioUNet$_S$ Estimation}
		\label{fig:radio2}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.32\textwidth}\centering
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/7_explanation2.png}
		\caption{Standard RadioUNet$_S$ Explanation}
	   \label{fig:radio3}
	\end{subfigure}%
	\hfill 
	\begin{subfigure}{0.32\textwidth}\centering
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/7_RadioUNet_C.png}
		\caption{RadioUNet$_C$ Estimation \newline}
	   \label{fig:radio4}
	\end{subfigure}%
	\hfill 
	\begin{subfigure}{0.32\textwidth}\centering
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/7_estimateT.png}
		\caption{Interpretation-Driven RadioUNet$_S$ Estimation}
	   \label{fig:radio5}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.32\textwidth}\centering
		\includegraphics[width=0.997\linewidth]{Figures/RadioMap/7_explanationT2.png}
		\caption{Interpretation-Driven RadioUNet$_S$ Explanation}
			\label{fig:radio6}
	\end{subfigure}%
	\caption{Radio map estimations and explanations. Gray: radio map. Blue: input buildings. Red: input measurements. Green: interpretation area of interest.}
	\label{fig:radio}
\end{figure}

\Ron{Remark: are apples comparable to oranges? How can I say that one building is comparable to one measurement as a piece of information? If the weights of buildings had corresponded to their area/norm then the relevance outcome would have been different. The currency between different types of information is in fact another part of the query.}


\subsection{Data}

\subsection{Model Architectures}

\subsection{Experiments}

\subsection{Results}

\subsection{MNIST Dataset (provisional)}

\subsubsection{Explanations}
In the following the results from the Experiments on MNIST using a 64-atom convolutional sparse dictionary.\\
The Pixel Space Max Reconstruction images show the following:\\
In the top there is a bar plot of the prediction of the classifier model. with the GT label written above.\\
In the lower left is the Digit as reconstructed from its sparse coding (This is very close to the original digit)\\
In the lower middle in blue, the maximum significance reconstruction is shown for all elements which have coefficient zero (in the sparse representation of the digit), i.e. which are not present in the image. So, in a sense, it is important for these features to be missing in the original image, or, in other words, it shows which elements, if added to the image, change the classification.\\
In the lower right in red, the maximum significance reconstruction is shown for all elements which have a non-zero coefficient. So in a sense, this shows which elements of the image have to be kept to preserve the classification.\\
\\
The significance maps for each component are composed as follows:\\
For each atom of the convolutional dictionary (shown in the 2nd, 4th, 6th and 8th column), its significance to the classification throughout the image is plotted on the left (1st, 3d, 5th, 7th column). As this is a convolutional dictionary, the significance map is coherent with the image plane, so a high value for example in the top left corner in the map indicates that the presence or absence of this particular atom in this top left region was important for the classification\\
Here, again blue pixels indicate that the corresponding coefficient is zero, i.e. that its important for the element to be missing in the image. \Ron{Perhaps pick one representative of each atom in each spatial patch, and plot just a few of the atoms in different colors so they can be identified individually. You can upscale the atoms smoothly to high resolution, threshold, and get a nice high definition shape. You can now also add high resolution contour. Then if you add some of these together (perhaps sum and not max?) at different colors they might be distinguishable.}
Red pixels on the other hand indicate that the corresponding coefficient is nonzero, i.e. that its important for this element to be present in this position in the image. \Ron{Same here, without the spatial representatives.}

\subsubsubsection{Correct classifications}
Pixel Space Max Reconstruction:\\
\includegraphics[scale=0.3]{Figures/MNISTImages/Example6_base.png}\\
Significance Maps for each component:\\
%\includegraphics[scale=0.15]{Figures/MNISTImages/Example6_smap.png}\\

Pixel Space Max Reconstruction:\\
\includegraphics[scale=0.3]{Figures/MNISTImages/Example8_base.png}\\
Significance Maps for each component:\\
%\includegraphics[scale=0.15]{Figures/MNISTImages/Example8_smap.png}\\

Pixel Space Max Reconstruction:\\
\includegraphics[scale=0.3]{Figures/MNISTImages/Example9_base.png}\\
Significance Maps for each component:\\
%\includegraphics[scale=0.15]{Figures/MNISTImages/Example9_smap.png}\\

\subsubsection{Incorrect classifications}
Pixel Space Max Reconstruction:\\
\includegraphics[scale=0.3]{Figures/MNISTImages/Example0_base.png}\\
Significance Maps for each component:\\
%\includegraphics[scale=0.15]{Figures/MNISTImages/Example0_smap.png}\\

Pixel Space Max Reconstruction:\\
\includegraphics[scale=0.3]{Figures/MNISTImages/Example2_base.png}\\
Significance Maps for each component:\\
%\includegraphics[scale=0.15]{Figures/MNISTImages/Example2_smap.png}\\

Pixel Space Max Reconstruction:\\
\includegraphics[scale=0.3]{Figures/MNISTImages/Example5_base.png}\\
Significance Maps for each component:\\
%\includegraphics[scale=0.15]{Figures/MNISTImages/Example5_smap.png}\\


\subsection{NSynth Dataset (provisional)}
\subsubsection{The Inpainter}
Example outputs from Inpainter for five different classes. Spectra are l2-normalized and sampled logarithmically between 20Hz and 8000Hz with 1024 samples.\\
\includegraphics[scale=0.3]{Figures/NSynthImages/InpainterOutNSynth.png}
Loss curve of the inpainter: (it has not converged yet)\\
\includegraphics[scale=0.31]{Figures/NSynthImages/loss_curve_gan.png}

\subsubsection{Explanations}
Optimized with Adam optimizer, 1e+6 steps, batch size of 8 (its so small to get more stochasticity in the inpainter), step size = 1e-4, $\lambda$ = 10. The quantity optimized is $$ \frac12 \mathbb{E}[(\Phi_d(x) - \Phi_d(z))^2] + \lambda ||s||_1 $$ over s with
$z = x  (1-s) + y s$ with $y$ being the inpainted input using a projection of $s$ onto $\{0,1\}^n$. Gradients are not propagated through the inpainter. $d$ is the dimension of the classifiers output with the highest activation.

\includegraphics[scale=0.3]{Figures/NSynthImages/input_and_s01.png}
\includegraphics[scale=0.3]{Figures/NSynthImages/input_and_s02.png}
\includegraphics[scale=0.3]{Figures/NSynthImages/input_and_s11.png}
\includegraphics[scale=0.3]{Figures/NSynthImages/input_and_s12.png}
\includegraphics[scale=0.3]{Figures/NSynthImages/input_and_s21.png}
\includegraphics[scale=0.3]{Figures/NSynthImages/input_and_s22.png}

==> sections/related.tex <==
\section{Related Work}

Our work is most similar to RDE\cite{DBLP:journals/corr/abs-1905-11092}. We use the same optimization target,
$$D(s) = \frac12 \mathbb{E}_{z \sim \Upsilon_{s}}[(\Phi_d(x) - \Phi_d(z))^2] + \lambda ||s||_1 $$

However, as explained in Sec~\ref{sec:method}, we improve the process by assuming access to the training dataset in order to make the choice of $z$ more rigorous through the novel use of an Inpainter $g$. Consequently, we can be confident that our masked data, after being funneled through the Inpainter, will be on the data distribution and thus the approach will now only say whether a selected region is important to the classification decision or not.

Another related work is LIME \cite{DBLP:journals/corr/RibeiroSG16}, which similarly assumes access to the training dataset and trains a new model on perturbed data. However, rather than make use of a discriminator that ensures we are close to the data distribution, they weight the resulting classification decisions according to how far the perturbed datum is from the original datum. Hence, they maintain a locally linear surrogate to the original model. Further, this approach suffers from the same concern that RDE has in that it yields the perturbations by randomly adjusting `superpixels' in order to train the surrogate. While this will likely not stray too far from the distribution because of the weighting, it is still a concern that the surrogate has a wider domain than the original model which may overstep the decision boundaries. In contrast, once we have trained our Inpainter, we have a much more founded tool with which to sample data that lets us decipher what was important towards the model's decision.

\cinjon{
TODO: talk about these deficiences of LIME and why we get aroudn it:
}
\cinjon{
In Lime, Sampling could be improved in the current implementation of LIME. Data points are sampled from a Gaussian distribution, ignoring the correlation between features. This can lead to unlikely data points which can then be used to learn local explanation models.
}
\cinjon{
The complexity of the explanation model has to be defined in advance. This is just a small complaint, because in the end the user always has to define the compromise between fidelity and sparsity. (we use the data distribution itself to govern the complexity)
}

Finally, there is a large class of approaches that are based on back-propagating through the network in order to produce a sensitivity analysis of which inputs were important \cite{10.1371/journal.pone.0130140,DBLP:journals/corr/ShrikumarGK17,Simonyan14a,DBLP:journals/corr/ZeilerF13}. Whereas our approach is model-agnostic, these methods can only be used on gradient-based neural networks. 


==> workshop/method.tex <==
\section{Method}
\label{sec:method}

We are given access to a black box model $\Phi$ and a target datum $x$ for which we would like to understand why the model considers $\Phi(x) = \hat{y}$. We alter some aspect of $x$ with a transformation $T(x) = x'$ in order to evaluate whether that aspect was important to the model's decision. This transformation $T$ is typically done by setting regions in the image to a background color\cite{DBLP:journals/corr/RibeiroSG16}, randomly flipping pixels\cite{DBLP:journals/corr/abs-1905-11092}, or by blurring specific regions\cinjon{cite}.

In this work, we build off of two papers. The first is \citet{DBLP:journals/corr/abs-1905-11092}, which evaluates whether $\Phi(x) = \Phi(x') = \hat{y}$ remains true after the transformation. It connects this with Rate-Distortion theory and formulates the task of interpreting the model as finding a partition of components of $x$ into relevant and irrelevant components $S$ and $S^c$. For a probability distribution $\Upsilon$ defined on $[0, 1]^d$, from which random vectors $n \sim \Upsilon$ are drawn, the obfuscation $z$ of $x$ wrt $S$ and $\Upsilon$ is defined by $z_S = x_S$ and $z_{S^c} = n_{S^c}$.
%\Ron{, where $w_S$ denotes the restrictions of the vector $w$ to the entries $S$? Or clarify that this is a generic notation that can have different meanings.}.
Labeling the resulting distribution as $\Upsilon_S$, we arrive at an expected distortion of $S$ wrt $\Phi$, $x$, and $\Upsilon$ referred to as Rate-Distortion Explanation (RDE):
\begin{align*}
D(S, \Phi, x, \Upsilon) = \frac12 \mathbb{E}_{z \sim \Upsilon_{S}}[(\Phi(x) - \Phi(z))^2]
\end{align*}
Similarly to how rate-distortion is used to analyze lossy data compression, RDE scores the components of $S$ according to the expected deviation from the original datum's classification score. The smallest set $S$ that ensures a limited distortion $D(S)$ will contain the most relevant components. Intuitively, this is finding a minimal set of components in $x$ which cannot be randomly changed without effecting $\Phi$'s classification, which are the components that we expect to be important. However, there is a subtle issue that reduces the effectiveness of this procedure that also affects other approaches like LIME \cite{DBLP:journals/corr/RibeiroSG16}.

The issue is that when we modify the image with random noise or setting parts of the image to a background color, we do not know if the obfuscation is still in the domain of $\Phi$. In other words, is $z$ close enough to the training data distribution for the minimization of the functional $D$ to give meaningful information about why $\Phi$ made its decisions? If it is not close enough, then it is difficult to say that the classifier made its decision because that particular set of components in $S$ were important or not. It may instead be because $z$ is in a region of space for which the model has never developed a sufficient decision boundary.

\citet{chang2018explaining} addresses this by training $T$ using an adversarial approach under the Generative Adversarial Network (GAN, \cite{Goodfellow2014GenerativeAN}) framework. This requires access to a training data distribution $\mathcal{D}$. There are circumstances where this is not possible, such as when examining a model packaged as part of a larger software installation, however we consider it to be a reasonable request in most scenarios.

While they then uses log-odds to measure the classifier's prediction, we rely on the above definition of distortion for rigor. Therefore, with $s \in [0, 1]^d$ 
%\Ron{The notations $s$ and $\theta$ are a bit confusing. You first assume that $s$ is soft, but then $\theta$ is the soft mask and $s$ is binary and sampled from $\theta$. So maybe assume  $s\in\{0,1\}$ from the beginning.} 
and the obfuscation $z = x \odot s + n \odot (1 - s)$, we follow \cite{DBLP:journals/corr/abs-1905-11092} and formalize the optimization approach as minimizing the following:
\begin{align*}
D(s) = \frac12 \mathbb{E}_{z \sim \Upsilon_{s}}[(\Phi_d(x) - \Phi_d(z))^2] + \lambda ||s||_1 
\end{align*}
\cosmas{We should use another D here also}

% The issue is that when we modify the image with random noise or setting parts of the image to a background color, we do not know if the obfuscation is still in the domain of $\Phi$. In other words, is $z$ close enough to the training data distribution for the minimization of the functional $D$ to give meaningful information about the mode of operation of $\Phi$? If it is not close enough, then we cannot justifiably say that the classifier made its decision because that particular set of components in $S$ were important or not. It may instead be because the obfuscation $z$ is in a region of space for which the model has never developed a sufficient decision boundary.

% To ground this concern, consider the colored MNIST setup from \citet{Arjovsky2019InvariantRM}. The goal is to predict a binary label of whether the seen number is less than five or greater than four. The images are colored either red or green in a way that correlates strongly with the class label. By construction, the label is more strongly correlated with the color than the digit, so an algorithm may learn to rely on the color or it may learn to rely on the digit, but the former is more likely. 

% For a model that learns to rely on the digit, then randomly turning pixels off will find the minimal important components as desired. But for a model that learns to rely on the color, this will not because \textit{any} of the pixels will be sufficient. The minimal set would be any pixel turned on. More importantly though, it would also be every other pixel \textit{not} turned to the opposite color. Without having an understanding of the data distribution, we would not be able to parse this apart. \textcolor{blue}{(Ron) I think that the problem is that every pixel will be transmitted, or at least most will, since otherwise non-transmitted pixels have random colors.}
% \cosmas{I don't know if we need this explanation. Maybe its just better to cite the paper that shows that because of this there are problems with LIME.}

The inpainting network $G$ then takes as input $x$, the mask $s$, and a noise vector $n$, and generates an output s.t.
\begin{align*}
\label{eq:z}
z(x, s, n) = x \odot s + G(x, s, n) \odot (1 - s)
\end{align*}
is on the distribution $\mathcal{D}$. This corresponds to training $G$ such that by sampling $n$, the resulting $z(x,s,n) \sim \mathcal{D}|_{z_S=x_S}$.

Note that we conceptually think of $s$ as a binary mask as it represents the partition of $x$ into $x_S$ and $x_{S^c}$. While the l1-regularization does encourage it to be a dirac, this property is not guaranteed due to it being a soft variable during optimization. To circumvent this, \cite{chang2018explaining} uses the concrete distribution \cite{DBLP:journals/corr/MaddisonMT16,jang2016categorical} and samples $s$ from the continuous relaxation of a Bernoulli variable with probability $\theta$. Optimizing $\theta$ yields the objective:
\begin{align*}
    \theta^* = \underset{\theta,\ s\sim\text{Bern}_\theta}{\text{argmin}} D(s).
\end{align*}
We can now use $G$ to sample from the conditional data distribution and then estimate $D(s)$ before optimizing $\theta$ with stochastic gradient descent. 
%Note here that the generative model $G$ does not necessarily have to allow for gradient backpropagation as gradients can be assigned to $s$ via \eqref{eq:z}.

% We train $G$ to inpaint via the GAN framework\cite{Goodfellow2014GenerativeAN,Pajot2019UnsupervisedAI,DBLP:journals/corr/abs-1801-07892,10.1145/3072959.3073659} where $G$ is the generator trying to fool a similarly powerful critic that tries to discriminate whether $z(x, s, n)$ came from the original distribution or from $G$. After convergence, we can then use $G$ alongside RDE in order to illuminate which components were important without running into the entangled distribution concern.

%In fact, we consider a more general setting, in which we minimize
%\begin{align*}
%E(s) = \frac12 \mathbb{E}_{z \sim \Upsilon_{s}}[(\Phi_d(x) - \Phi_d(z))^2] + \lambda ||s||_1 
%\end{align*}



\Ron{We can formulate the greedy algorithm probabilistically. In the greedy algorithm we add sequentally more and more conditions in the conditional probability. At step $n+1$ we have chosen the features $f_1,\ldots, f_n$. We then find a feature $f_{n+1}$ for which the mean classification error (distance from the original classification outcome) of the random variable $( x | f_1,\ldots, f_{n+1})$ is minimal. This random variable hase probability distribution $P( x | f_1,\ldots, f_{n+1})$ implicitly given by the inpainter (the generative model), and we use Monte Carlo to estimate the mean error.} 

%  In RDE, $$z = x \odot s + n \odot (1 - s)$$ where $n\sim\Upsilon$ and $\Upsilon$ is a normal distribution. With this approach, if the classifier decides that $z$ results in another class, then it is not clear whether this is because the pixels selected for removal by the mask were important or because $z$ is far from the data distribution. In the latter case, we should not expect the classifier to return anything reasonable, which obfuscates our ability to interpret the importance of a particular pixel. We fix this concern by making novel use of an Inpainting network trained on the data distribution such that 



% \subsection{GAN for inpainting and generation}
% For our method, the utilization of GANs is key for obtaining data completions which are feasible within the data distribution.\\
% In a sense our Generators are a mixture of inpainting models and generators as already used in many fields \memo{cite}.\\
% A major characteristic of this is a high amount of down and subsequent upsampling, the addition of noise vectors in the input and the deep features and skip connections \memo{this sentence should be written differently}.
